A Simple Recipe for Contrastively Pre-training Video-First Encoders Beyond 16 Frames

Understanding long, real-world videos requires modeling of long-range visual dependencies. To this end, we explore video-first architectures, building on the common paradigm of transferring large-scale, image--text models to video via shallow temporal fusion. However, we expose two limitations to the approach: (1) decreased spatial capabilities, likely due to poor video--language alignment in standard video datasets, and (2) higher memory consumption, bottlenecking the number of frames that can be processed. To mitigate the memory bottleneck, we systematically analyze the memory/accuracy trade-off of various efficient methods: factorized attention, parameter-efficient image-to-video adaptation, input masking, and multi-resolution patchification. Surprisingly, simply masking large portions of the video (up to 75%) during contrastive pre-training proves to be one of the most robust ways to scale encoders to videos up to 4.3 minutes at 1 FPS. Our simple approach for training long video-to-text models, which scales to 1B parameters, does not add new architectural complexity and is able to outperform the popular paradigm of using much larger LLMs as an information aggregator over segment-based information on benchmarks with long-range temporal dependencies (YouCook2, EgoSchema).

==> sec/temp_file.tex <==
\section{Introduction}
\label{sec:intro}

Although prior work has explored video pre-training in smaller-scale networks~\citep[\eg,][]{zellers2021merlot,fu2021violet,wang2022internvideo}, the prevailing paradigm for training video-to-text models includes several steps of training and depends on large language models (LLMs) for conditional generation~\citep[\eg,][]{alayrac2022flamingo,li2023blip, yang2022zero,ye2023mplug}.
This allows to first train powerful vision encoders and then harness the reasoning and generation powers of LLMs. 
Problematically though, recent approaches transfer large-scale image-to-text models to the video domain by tuning shallow modules performing late temporal fusion while keeping the pre-trained image encoder frozen~\cite{alayrac2022flamingo,yan2022video,ye2023mplug}. 
They test such approaches on short video benchmarks, which mostly contain limited temporal dependencies, and restrict the models to use a small number (8 to 16) of input frames. 
Finally, for scaling video-to-text models to longer sequences of frames, recent work explores modular approaches, where short video- or image-to-text models are used for captioning parts of the longer video and then LLMs are responsible for aggregating and composing information in order to address the downstream task~\cite{zeng2022socratic,li2023videochat,lin2023mmvid}.

In this paper, we explore video-first models for text-video retrieval and video-to-text generation which we scale to longer sequences of frames. We first contrastively pre-train a video encoder on a mixture of image and video data and then plug it into a pre-trained frozen LM for addressing video-to-text generation (video captioning, question answering) similarly to ~\citep{alayrac2022flamingo}.
We demonstrate that video-first encoders (Video ViT; ViViT~\cite{arnab2021vivit}) significantly improve performance over frame-level encodings on benchmarks with rich temporal dependencies, although this comes at a cost. For one, spatial capabilities of contrastively pre-trained video-first models decrease possibly due to the noisy video-text alignment and coarse-grained CLIP-style objective~\cite{luo2022clip4clip} which is better suited for images. Moreover, ViViT is memory hungry and difficult to scale to longer sequences of frames as compute and memory increase exponentially with the input length. For addressing the latter, we explore memory efficient adaptation methods, including input sampling, factorized attention, and parameter-efficient image-to-video adaptation, for scaling video-first models to longer sequences within a memory budget.

By evaluating first on text-video retrieval, we find that image-to-video adaptation fails to transfer spatial-only knowledge to the temporal dimension. Joint space-time attention in ViViT remains surprisingly robust to high input masking up to 75\% during contrastive training and offers 2-3x memory savings. 
In contrast, using different backbones, such as frame-level encodings or factorized attention, cannot maintain the same robustness against noisy video inputs and performance deteriorates further. 
Although Adapters~\cite{houlsby2019parameter} and semi-frozen tuning are incapable to transform image models to video-first, they can successfully adapt video models trained on short context (e.g., 16 seconds of video) to much longer temporal dependencies (videos up to 4.3 minutes).

We test vanilla and efficient variants of our short video models on text-video retrieval and video captioning on short video benchmarks (MSR-VTT~\cite{xu2016msr}, VATEX~\cite{wang2019vatex}, YouCook2~\cite{zhou2018towards}, and ActivityNet Captions~\cite{krishna2017dense}). We verify that image-based models are not enough for addressing tasks with rich temporal dependencies (e.g., YouCook2, VATEX). Our models are able to reach and in some cases surpass the performance of image-based VideoCoCa~\cite{yan2022video}.

We finally extend our short video model to longer contexts (LongViViT) of 256 frames (or 65.5k visual tokens) by further training on longer videos. We use the full-length videos of HowTo100M~\cite{miech2019howto100m} accompanied by LLM-generated summaries based on the ASR to further train the video encoder while masking 75\% of the input video tokens and freezing part of the network.
Our LongViViT-to-text model, which accounts for less than 1B parameters, outperforms modular methods that use LLM assistance (Bard-25B) and PALI-5B for frame captioning on temporally rich benchmarks (YouCook2, EgoSchema). Even modular methods that consider frame selection (SeViLA~\cite{yu2023self}) or an oracle segmentation of the video for short video captioning (for YouCook2) are not able to reach LongViViT's performance.
Our results highlight the importance of learning to encode longer-range contexts in videos. LLMs are powerful for reasoning, summarizing content, and answering to questions, but if we suboptimally encode the visual context, we might suffer from irreversible information loss depending on the benchmark.


In this paper, we explore best practices for pre-training video-language models with video-first architectures in contrast to the current paradigm of transferring frozen image encoders to videos via late temporal fusion. Evaluating on popular short video benchmarks (MSR-VTT, YouCook2, VATEX, ActivityNet Captions, EgoSchema), we find that video-first models pre-trained further on the video domain yield improvements in datasets with strong temporal dependencies. However, we expose two limitations to the approach: (1) decreased spatial capabilities, likely due to noisy video-language alignments and too coarse-grained objectives and (2) higher memory consumption, bottlenecking the number of frames that can be processed. 

To mitigate the memory bottleneck, we explore ways to improve memory efficiency in video encoders via input sampling, parameter-efficient image-to-video adaptation, or factorized attention. 

We find that just masking very high percentages of the input during training can improve memory consumption by 2-3x without drastically compromising performance. Using our techniques, we scale the memory-efficient video encoders to 256 frames (65.5k visual tokens), and test them against the popular paradigm of using a strong LLM-based information aggregation approach~\cite{zeng2022socratic,li2023videochat,lin2023mmvid}. We report results on the full-length videos of YouCook2, ActivityNet Captions (video summarization) and EgoSchema (video question-answering), and find that encoding the entire video is beneficial for benchmarks with long-range temporal dependencies (YouCook2, EgoSchema).

In this paper, we explore best practices for pre-training video-language models with video-first architectures in contrast to the current paradigm of transferring frozen image encoders to videos via late temporal fusion. Evaluating on popular short video benchmarks (MSR-VTT, YouCook2, VATEX, ActivityNet Captions, EgoSchema), we find that video-first models pre-trained further on the video domain yield improvements in datasets with strong temporal dependencies. However, we expose two limitations to the approach: (1) decreased spatial capabilities, likely due to noisy video-language alignments and too coarse-grained objectives and (2) higher memory consumption, bottlenecking the number of frames that can be processed. To mitigate the memory bottleneck, we explore ways to improve memory efficiency in video encoders via input sampling, parameter-efficient image-to-video adaptation, or factorized attention. We find that just masking very high percentages of the input during training can improve memory consumption by 2-3x without drastically compromising performance. Using our techniques, we scale the memory-efficient video encoders to 256 frames (65.5k visual tokens), and test them against the popular paradigm of using a strong LLM-based information aggregation approach~\cite{zeng2022socratic,li2023videochat,lin2023mmvid}. We report results on the full-length videos of YouCook2, ActivityNet Captions (video summarization) and EgoSchema (video question-answering), and find that encoding the entire video is beneficial for benchmarks with long-range temporal dependencies (YouCook2, EgoSchema).


In contrast to recent work that transfers larger-scale image-to-text models to the video domain via shallow late temporal fusion while keeping the image encoder frozen, we train video-first encoders, plug them into a frozen LM, and demonstrate that utilizing joint space-time attention yields improvements on benchmarks with strong temporal dependencies (YouCook2, VATEX). However, we expose two limitations to the approach: (1) decreased spatial capabilities, likely due to noisy video-language alignments and (2) higher memory consumption, bottlenecking the number of frames that can be processed. To mitigate the memory bottleneck, we systematically analyze ways to improve memory efficiency in video encoders via input sampling, parameter-efficient image-to-video adaptation, or factorized attention. Surprisingly, just masking large portions of the video (up to 75\%) proves to be the most robust way to scale encoders to videos up to 4.3 minutes at 1 fps rate. Our simple approach for training long video-to-text models that account for less than 1B parameters is able to outperform the popular paradigm of using a strong LLM as information aggregator over segment-based information~\cite{zeng2022socratic,li2023videochat,lin2023mmvid} on benchmarks with long range temporal dependencies (YouCook2, ActivityNet, EgoSchema).


